Generalize Your Face Forgery Detectors: An Insertable Adaptation Module Is All You Need

A plethora of face forgery detectors exist to tackle facial deepfake risks. However, their practical application is hindered by the challenge of generalizing to forgeries unseen during the training stage. To this end, we introduce an insertable adaptation module that can adapt a trained off-the-shelf detector using only online unlabeled test data, without requiring modifications to the architecture or training process. Specifically, we first present a learnable class prototype-based classifier that generates predictions from the revised features and prototypes, enabling effective handling of various forgery clues and domain gaps during online testing. Additionally, we propose a nearest feature calibrator to further improve prediction accuracy and reduce the impact of noisy pseudo-labels during self-training. Experiments across multiple datasets show that our module achieves superior generalization compared to state-of-the-art methods. Moreover, it functions as a plug-and-play component that can be combined with various detectors to enhance the overall performance.

==> tabs/insertable_test.tex <==
\begin{table}[tb!]
  \centering
  \scalebox{0.95}{
  \begin{tabular}{c|c|c|c|c|c} \toprule
    Method & Eff-b4 & SRM & SPSL & Recce & F3Net \\ 
    \midrule
    Baseline  & 0.749 & 0.755 & - & - & - \\
    % w/ Our module CDF  & \textbf{0.762} & \textbf{-} & \textbf{-} & \textbf{-} & -\\
    % w/ Our module DFD  & \textbf{0.762} & \textbf{-} & \textbf{-} & \textbf{-} & -\\
    % w/ Our module DFDC  & \textbf{0.762} & \textbf{-} & \textbf{-} & \textbf{-} & -\\
    w/ Our module  & \textbf{0.856} & \textbf{0.840} & \textbf{0.810} & \textbf{-} & -\\
    \bottomrule
  \end{tabular}
  }
  \caption{
  Ablation studies of different base detectors.
  }
  \label{tab:ablation_insertable}
  \vspace{-1pt}
\end{table}
